Identification and Removal of Noise Modes in Kepler Photometry

We present the Transiting Exoearth Robust Reduction Algorithm (TERRA) --- a novel framework for identifying and removing instrumental noise in Kepler photometry. We identify instrumental noise modes by finding common trends in a large ensemble of light curves drawn from the entire Kepler field of view. Strategically, these noise modes can be optimized to reveal transits having a specified range of timescales. For Kepler target stars of low photometric noise, TERRA produces ensemble-calibrated photometry having 33 ppm RMS scatter in 12-hour bins, rendering individual transits of earth-size planets around sun-like stars detectable as ~3 sigma signals.

==> abundhist.tex <==
$ {[}O/H] $& 694 & 0.06 & 0.14 & -0.91 & 0.43\\$ {[}C/H] $& 704 & 0.09 & 0.17 & -0.52 & 0.52\\$ {[}Fe/H] $& 1070 & 0.07 & 0.27 & -1.95 & 0.56\\

==> changes.tex <==
diff --git a/manuscript.tex b/manuscript.tex
index 85a94bb..8110cb3 100644
--- a/manuscript.tex
+++ b/manuscript.tex
@@ -43,7 +43,7 @@
 \keywords{techniques: photometric --- planetary systems}
 
 \begin{abstract}
-We present the Transiting Exoearth Robust Reduction Algorithm (TERRA) --- a novel framework for identifying and removing instrumental noise in \Kepler photometry.   We identify instrumental noise modes by finding common trends in a large ensemble of light curves.  Our approach is novel in the sense that our mode construction is optimized for transit-length timescales.  We produce corrected photometry with a simpler and more robust noise model than the Pre-search Data Conditioning (PDC) algorithm of \cite{Twicken:2010}, which attempts to remove systematic noise at all timescales.  For the low noise stars that are most amenable to exoearth detection, TERRA achieves an additional 10~ppm suppression of instrumental noise with timescales comparable to the $\sim$10~hour transit of an earth-sized planet at 1 AU.
+We present the Transiting Exoearth Robust Reduction Algorithm (TERRA) --- a novel framework for identifying and removing instrumental noise in \Kepler photometry.   We identify instrumental noise modes by finding common trends in a large ensemble of light curves.  Our approach is novel in the sense that our mode construction is optimized for transit-length timescales.  TERRA offers advantages in some special regimes of signal detection compared to the Pre-search Data Conditioning (PDC) algorithm of \cite{Twicken:2010}, which attempts to remove systematic noise at all timescales.  For the low noise stars that are most amenable to exoearth detection, TERRA achieves an additional 10~ppm suppression of instrumental noise with timescales comparable to the $\sim$10~hour transit of an earth-sized planet at 1 AU.
 \end{abstract}
 
 \section{Introduction}
@@ -61,9 +61,7 @@ We present the Transiting Exoearth Robust Reduction Algorithm (TERRA) --- a fram
 
 \section{Instrumental Noise in \Kepler Photometry}
 \label{sec:InstNoise}
-There are many sources of noise in \Kepler photometry other than Poisson shot noise. Since many of these noise sources are coherent on timescales longer than one cadence (29.4~minutes), the scatter in $N_{C}$ bins does not decrease as $1/\sqrt{ N_{C} }$.  Thus, photometric noise is a function of bin size.  The \Kepler team computes a quantity called CDPP12 which is a measure of the photometric scatter in 12-hour bins.  We illustrate some of these noise sources with the Simple Aperture Photometry (SAP) from KIC-8144222 (\Kmag = 12.4, CDPP12 = 35.4 ppm) shown in Figure~\ref{fig:SampLC}.  The dominant systematic effect on multi-quarter timescales is ``differential velocity aberation'' \citep{VanCleve:2009}.  As \Kepler orbits the sun, its velocity relative to the \Kepler field changes.  When the spacecraft approaches the \Kepler field, stars on the extremities of the field move toward the center.  Stellar PSFs move over \Kepler apertures by $\sim$ 1 arcsecond resulting in a $\sim$ 1 \% effect over 1-year timescales.
-
-We show a detail of KIC-8144222 photometry from Quarter 6 (Q6) in Figure~\ref{fig:SampLC}.  As a comparison, we randomly selected three stars, which were similar to KIC-8144222 in position on the Field of View (FOV), noise level, and brightness (mod.out = 16.1, CDPP12 $<$ 40 ppm, 12.0 $<$ \Kmag $<$ 13.0).  We show their light curves in Figure~\ref{fig:SampLC}, and it is clear that much of the variability is correlated and hence, due to the state of the \Kepler spacecraft.  The decaying exponential shapes are caused by thermal settling.  There is also a $\sim$0.1\% effect with a 3-day period due to thermal coupling of telescope optics to the reaction wheels, which we explore in depth in \S~\ref{sec:interpretation}.  Since both of these effects are intrinsic to the \Kepler spacecraft and not to KIC-8144222, we see the same effects in other stars.  Common trends among stars can be identified and removed.  The \Kepler team calls this ``cotrending,'' a term which we adopt.  For a more complete description of noise in \Kepler data see \cite{Christiansen:2011}.
+The \Kepler spacecraft makes photometric observations of $\sim$156,000 targets.  Long cadence photometry is computed by summing all the photoelectrons within a predefined target aperture during a 29.4~minute integration.  The \Kepler team makes this ``Simple Aperture Photometry'' available to the scientific community~\citep{KeplerArchiveManual}.  Simple aperture photometry contains many sources of noise other than Poisson shot noise.  We illustrate several noise sources in Figure~\ref{fig:SampLC}, where we show the normalized photometry ($\df$) of KIC-8144222 (\Kmag = 12.4).  $\df = (F-\overline{F})/\overline{F}$ where $F$ is the simple aperture photometry.
 
 \begin{figure}[htbp]
 \begin{center}
@@ -73,10 +71,18 @@ We show a detail of KIC-8144222 photometry from Quarter 6 (Q6) in Figure~\ref{fi
 \end{center}
 \end{figure}
 
-Correlated noise with timescales between 1 and 10 hours can mimic planetary transits and requires careful treatment.  To illustrate the transit-scale correlations among a large sample of stars, we show a correlation matrix constructed from 200 Q6 light curves in Figure~\ref{fig:corrmat} organized by module.  We constructed the correlation matrix using the following steps:
+The dominant systematic effect on multi-quarter timescales is ``differential velocity aberration'' \citep{VanCleve:2009}.  As \Kepler orbits the sun, its velocity relative to the \Kepler field changes.  When the spacecraft approaches the \Kepler field, stars on the extremities of the field move toward the center.  Stellar PSFs move over \Kepler apertures by $\sim$ 1 arcsecond resulting in a $\sim$ 1 \% effect over 1-year timescales.
+
+We show a detailed view of KIC-8144222 photometry from Quarter 6 (Q6) in Figure~\ref{fig:SampLC}.  The decaying exponential shapes are caused by thermal settling after data downlinks.  Each month, \Kepler rotates to orient its antenna toward earth.  Since \Kepler is not a uniformly colored sphere, changing the spacecraft orientation with respect to the sun changes its overall temperature.  After data downlink, \Kepler takes several days to return to its equilibrium temperature (Jeffrey Smith, private communication, 2012).  KIC-8144222 photometry also shows a $\sim$0.1\% effect with a 3-day period due to thermal coupling of telescope optics to the reaction wheels.  We explore this 3-day cycle in depth in \S~\ref{sec:interpretation}.
+
+Since all of the previously mentioned noise sources are coherent on timescales longer than one cadence (29.4~minutes), the RMS of binned photometry does not decrease as $1/\sqrt{N}$, where N is the number of measurements per bin.  In order to describe the noise on different timescales, the \Kepler team computes quantities called CDPP3, CDPP6, and CDPP12 which are measures of the photometric scatter in 3, 6, and 12-hour bins.  KIC-8144222 has CDPP12 35.4~ppm and is a low-noise star (bottom 10 percentile).  For a more complete description of noise in \Kepler data see \cite{Christiansen:2011}.
+
+As a comparison, we selected stars which were similar to KIC-8144222 in position on the Field of View (FOV), noise level, and brightness (mod.out = 16.1, CDPP12 $<$ 40 ppm, 12.0 $<$ \Kmag $<$ 13.0).  From this 13-star sample, we randomly selected 3 stars and show their light curves in Figure~\ref{fig:SampLC}.  The photometry from the comparison stars is strikingly similar to the KIC-8144222 photometry.  Since much of the variability is correlated, it must be due to the state of the \Kepler spacecraft.  Common trends among stars can be identified and removed.  The \Kepler team calls this ``cotrending,'' a term we adopt.  
+
+Correlated noise with timescales between 1 and 10 hours can mimic planetary transits and requires careful treatment.  To illustrate the transit-scale correlations among a large sample of stars, we show a correlation matrix constructed from 200 Q6 light curves in Figure~\ref{fig:corrmat}.  The \Kepler photometer is an array of 42 CCDs arranged in 21 modules~\citep{KeplerArchiveManual}.  We organized the rows and columns of the correlation matrix by module.  We constructed the correlation matrix using the following steps:
 \begin{enumerate}
 \item
-We randomly selected 10 light curves from each of the 20 total modules from stars with the following properties: $12.5 < $ \Kmag $ < 13.5$ and CDPP12 $< 40$~ppm.  
+We randomly selected 10 light curves from each of the 20 total modules\footnote{Module 3 failed during Q4~\citep{Christiansen:2011}.} from stars with the following properties: $12.5 < $ \Kmag $ < 13.5$ and CDPP12 $< 40$~ppm.  
 \item
 To highlight transit-scale correlations, we subtracted a best fit spline from the photometry.  The knots of the spline are fixed at 10-day intervals so that we remove trends $\gtrsim$ 10~days.
 \item
@@ -84,7 +90,7 @@ We normalized each light curve so that its median absolution deviation (MAD) is
 \item
 We evaluated the pairwise correlation (Pearson-R) between all 200 stars.  
 \end{enumerate}
-The correlation matrix shows that stars are highly correlated with other stars in the same module.  However, the large off-diagonal correlations show there is significant intra-module correlation.
+The correlation matrix shows that stars in some modules (e.g. module 2)correlate strongly with other stars in the same module.  However, other modules (e.g. module 12) shows little inter-module correlation.  Finally, the large off-diagonal correlations show that stars in some modules correlate strongly with stars in different modules.  
 
 \begin{figure}[htbp]
 \begin{center}
@@ -99,13 +105,14 @@ The correlation matrix shows that stars are highly correlated with other stars i
 We have shown that there is significant high-frequency ($\lesssim$ 10~days) systematic noise in \Kepler photometry.  In order to recover the smallest planets, this noise must be carefully characterized and removed.  We isolate systematic noise by finding common trends in a large ensemble of stars.  This is an extension of differential photometry, widely used by ground-based transit surveys to calibrate out the time-variable effects of the earth's atmosphere.  We find these trends using Principle Component Analysis (PCA).  This is similar to the Sys-Rem, TFA, and PDC algorithms \citep{Tamuz:2005,Kovacs:2005,Twicken:2010}, but our implementation is different.  We briefly review PCA in the context of cotrending a large ensemble of light curves.
 
 \subsection{PCA on Ensemble Photometry}
-Consider an ensemble of N light curves each with M cadences.  We can think of the ensemble as a collection of N points in an M-dimensional space.  Each light curve $\df$ can be written as a linear combination of M basis vectors that span the space.  
-\begin{eqnarray*}
-\df_{1} & = & a_{1,1} V_1 + \hdots  +  a_{1,M} V_M \\
+Consider an ensemble of N light curves each with M photometric measurements.  We can think of the ensemble as a collection of N vectors in an M-dimensional space.  Each light curve $\df$ can be written as a linear combination of M basis vectors that span the space,  
+\begin{eqnarray}
+\label{eqn:BV}
+\df_{1} & = & a_{1,1} V_1 + \hdots  +  a_{1,M} V_M \notag\\
         &\vdots&\\
-\df_{N} & = & a_{N,1} V_1 + \hdots  +  a_{N,M} V_M \\
-\end{eqnarray*}
-or more compactly as
+\df_{N} & = & a_{N,1} V_1 + \hdots  +  a_{N,M} V_M \notag
+\end{eqnarray}
+where each of the $V_{j}$ basis vectors is the same length as the original photometric time series.  Equation~\ref{eqn:BV} can be written more compactly as
 \[
 \mtx{D} = \mtx{A} \mtx{V}
 \]
@@ -130,13 +137,13 @@ where
   V_{M} \\
 \end{pmatrix}
 \]
-Singular Value Decomposition (SVD) simultaneously solves for the basis $\mtx{V}$ and the coefficient matrix $\mtx{A}$ because it decomposes any matrix $\mtx{D}$ into
+Singular Value Decomposition (SVD) simultaneously solves for the basis vectors $\mtx{V}$ and the coefficient matrix $\mtx{A}$ because it decomposes any matrix $\mtx{D}$ into
 \[
-\mtx{D} = \mtx{USV}.
+\mtx{D} = \mtx{USV}^{\mathsf{T}}.
 \]
-$\mtx{V}$ is an M x M matrix where the rows are the eigenvectors of $\mtx{D}^{T}\mtx{D}$ or ``principle components,'' and the diagonal elements of S are the corresponding eigenvalues.  The eigenvalues $\{s_{1,1}, \dots, s_{M,M}\}$ describe the extent to which each of the principle components capture variability in the ensemble and are ordered from high to low.  
+$\mtx{V}$ is an M x M matrix where the columns are the eigenvectors of $\mtx{D}^{\mathsf{T}}\mtx{D}$ or ``principle components,'' and the diagonal elements of S are the corresponding eigenvalues.  The eigenvalues $\{s_{1,1}, \dots, s_{M,M}\}$ describe the extent to which each of the principle components capture variability in the ensemble and are ordered from high to low.  The columns of $\mtx{U}$ are the eigenvectors of  $\mtx{D}\mtx{D}^{\mathsf{T}}$.  Both $\mtx{U}$ and $\mtx{V}$ are unitary matrices, i.e. $\mtx{U}\mtx{U}^{\mathsf{T}} = \mtx{I}$ and $\mtx{V}\mtx{V}^{\mathsf{T}} = \mtx{I}$.
 
-As we saw in \S~\ref{sec:InstNoise}, most of the variability is correlated among stars, so we expect the first principle components to correspond to the instrumental noise modes we are trying to remove.  If we identify the first $N_{Mode}$ principle components as instrumental noise modes, we can remove them via
+As we saw in \S~\ref{sec:InstNoise}, stars show common photometric trends due to changes in the state of the \Kepler spacecraft.  The most significant principle components will correspond to these common trends.  If we identify the first $N_{Mode}$ principle components as instrumental noise modes, we can remove them via
 \begin{equation}
 \df_{i,cal} = \df_{i} - \sum_{j=1}^{N_{Mode}} a_{i,j} V_{j}
 \label{eqn:fit}
@@ -144,9 +151,9 @@ As we saw in \S~\ref{sec:InstNoise}, most of the variability is correlated among
 where $\df_{cal}$ is an ensemble-calibrated light curve.  However since the collection of $\{V_{i}, \hdots V_{M}\}$ spans the space, the higher principle components describe astrophysical variability, shot noise, and exoplanet transits.  We must be careful not to remove too many components because we would be removing the signals of interest.
 
 \subsection{PCA implementation}
-A major component of the PDC is the suppression of correlated trends in photometry.  As a point of reference, we briefly describe how PDC cotrends photometry (for a more complete picture see \citealp{Christiansen:2011}).  For every output channel (mod.out) the \Kepler team identifies the 50\% most correlated stars as a reference ensemble.  Then, the team performs a Singular Value Decomposition (SVD) of the ensemble light curves.  The principle components are called co-trending basis vectors (CBVs) and are available online.\footnote{http://archive.stsci.edu/Kepler/cbv.html}  One can fit out the instrumental systematics by solving for the optimum linear combination of CBVs.
+A major feature of the PDC algorithm is the suppression of correlated trends in photometry.  As a point of reference, we briefly describe how PDC cotrends photometry (for a more complete picture see \citealp{Christiansen:2011}).  Each of \textit{Kepler's} 42 CCDs is divided into 2 output channels.  For every output channel the \Kepler team identifies the 50\% most correlated stars as a reference ensemble.  Then, the team performs a Singular Value Decomposition (SVD) of the light curve ensemble.  The principle components are called co-trending basis vectors (CBVs) and are available online.\footnote{http://archive.stsci.edu/Kepler/cbv.html}  One can fit out the instrumental systematics by solving for the optimum linear combination of CBVs.
 
-We also use SVD to compute modes but our implementation is different.  We construct a large reference ensemble of light curves $\{\df_{1}, \dots, \df_{N}\}$ of 1000 stars ($12.5 < $ \Kmag $ < 13.5$, CDPP12 $< 40$~ppm) drawn randomly from the entire FOV.  Before performing SVD, we remove thermal settling events and trends $\gtrsim$ 10~days as described in \S~\ref{sec:InstNoise}.  Since SVD finds the eigenvectors of $\mtx{D}^{T}\mtx{D}$ it is susceptible to outliers like any least-squares estimator.  We perform a robust SVD that relies on iterative outlier rejection following these steps:
+We also use SVD to compute modes but our implementation is different.  We construct a large reference ensemble of light curves $\{\df_{1}, \dots, \df_{N}\}$ of 1000 stars ($12.5 < $ \Kmag $ < 13.5$, CDPP12 $< 40$~ppm) drawn randomly from the entire FOV.  Before performing SVD, we remove thermal settling events and trends $\gtrsim$ 10~days as described in \S~\ref{sec:InstNoise}.  Since SVD finds the eigenvectors of $\mtx{D}^{\mathsf{T}}\mtx{D}$ it is susceptible to outliers as is any least squares estimator.  We perform a robust SVD that relies on iterative outlier rejection following these steps:
 %
 \begin{enumerate}
 \item
@@ -163,29 +170,29 @@ Remove outlier light curves from the ensemble.
 Repeat until no outliers remain.
 \end{enumerate}
 %
-For our 1000-star sample we identified and removed 51 stars from our ensemble.  These stars tended to have high amplitude intrinsic variability.
+For our 1000-star sample we identified and removed 51 stars from our ensemble.  These stars tended to have high amplitude intrinsic astrophysical variability, i.e. due to spots and flares.
 
-We plot the four most significant TERRA principle components in Figure~\ref{fig:CompCBV} and compare them to the PDC CBVs.  We cleanly isolate the three-day cycle in the first principle component.  In contrast, this cycle appears in CBVs 2 and 3 and to a lesser extent in CBVs 1 and 4.  All of the PDC CBVs show $\gtrsim$10~day trends, as well as features due to thermal settling events.  This means that DVA and thermal settling affect photometry in a complex fashion, requiring many linearly independent components.  Modeling these trends requires higher model complexity, which can result in overfitting.  We circumvent this additional complexity by notching out thermal settling events and removing DVA with a simple spline. 
+We plot the four most significant TERRA principle components in Figure~\ref{fig:CompCBV} and compare them to the PDC CBVs.  We cleanly isolate the three-day cycle in the first principle component.  In contrast, this cycle appears in CBVs 2 and 3 and to a lesser extent in CBVs 1 and 4.  All of the PDC CBVs show $\gtrsim$10~day trends, as well as features due to thermal settling events.  This means that differential velocity aberration and thermal settling affect photometry in a complex fashion, requiring many linearly independent components.  Modeling these trends requires higher model complexity, which can result in overfitting.  We circumvent this additional complexity by notching out thermal settling events and removing differential velocity aberration with a simple spline. 
 
 \begin{figure}
 \begin{center}
 \includegraphics{CompCBV.pdf}
 \end{center}
 \caption{
-Top: The first four TERRA principle components in our 1000-light curve ensemble plotted in order of significance.  $V_{1}$ has a 3-day periodicity and is due to changes in the thermal state of the spacecraft caused by a 3-day momentum management cycle.  $V_{2}$ has a high frequency component (P = 1.68~hours) that could be due to a 20~minute thermal cycle from an onboard heater aliased with the 29.4~minute observing cadence  alias of a 20-minute thermal cycle driven by an onboard heater. Bottom: First four PDC CBVs. Structure due to DVA and thermal settling appears in all CBVs.  These effects couple to the photometry in a complex fashion, require many linearly independent basis vectors.  By removing them before performing SVD, TERRA greatly simplifies the noise model.
+Top: The first four TERRA principle components in our 1000-light curve ensemble plotted in order of significance.  $V_{1}$ has a 3-day periodicity and is due to changes in the thermal state of the spacecraft caused by a 3-day momentum management cycle.  $V_{2}$ has a high frequency component (P = 1.68~hours) that could be due to a 20~minute thermal cycle from an onboard heater aliased with the 29.4~minute observing cadence  alias of a 20-minute thermal cycle driven by an onboard heater. Bottom: First four PDC CBVs. Structure due to differential velocity aberration and thermal settling appears in all CBVs.  These effects couple to the photometry in a complex fashion, require many linearly independent basis vectors.  By removing them before performing SVD, TERRA greatly simplifies the noise model.
 }
 \label{fig:CompCBV}
 \end{figure}
 
 \subsection{Interpretation of Photometric Modes}
 \label{sec:interpretation}
-In this section, we associate the variability captured in the principle components to changes in the state of the \Kepler spacecraft that couple to photometry.  The three-day cycle isolated in our first principle component is due to a well-known, three-day momentum management cycle on the spacecraft \citep{Christiansen:2011}.  To keep a fixed position angle, \Kepler must counteract external torques by spinning up reaction wheels.  These reaction wheels have frictional losses which leak a small amount of heat into the spacecraft, which changes the PSF width of the stars.  
+In this section, we associate the variability captured in the principle components to changes in the state of the \Kepler spacecraft that couple to photometry.  The three-day cycle isolated in our first principle component is due to a well-known, three-day momentum management cycle on the spacecraft \citep{Christiansen:2011}.  To keep a fixed position angle, \Kepler must counteract external torques by spinning up reaction wheels.  These reaction wheels have frictional losses which leak a small amount of heat into the spacecraft, which changes the PSF width and shape of the stars.  
 
-We can gain a more detailed understanding of this effect, by examining how the mode weights corresponding to $V_{1}$, i.e. $\{a_{1,1}, \dots, a_{N,1} \}$, vary across the FOV.  We display the RA and Dec positions of our 1000-star sample in Figure~\ref{fig:RADecCoeff} and color-code the points with the value of $a_{i}$.  The $a_{1}$ and $a_{2}$ mode weights show remarkable correlation across the FOV.  That $a_{1}$ is positive in the center of the FOV and negative at the edges of the FOV means these two regions respond to the momentum cycle in an anticorrelated sense.  The telescope is focused such that the PSF is sharpest at intermediate distances from the center of the FOV.  Since stars in the center and on the extreme edges have the blurriest PSFs \citep{VanCleve:2009}, they respond the strongest to the momentum cycle. 
+We can gain a more detailed understanding of this effect, by examining how the mode weights for each reference star corresponding to $V_{1}$, i.e. $\{a_{1,1}, \dots, a_{N,1} \}$, vary across the FOV.  We display the RA and Dec positions of our 1000-star sample in Figure~\ref{fig:RADecCoeff} and color-code the points with the value of $a_{i}$.  The $a_{1}$ and $a_{2}$ mode weights show remarkable spatial correlation across the FOV.  That $a_{1}$ is positive in the center of the FOV and negative at the edges of the FOV means the systematic photometric errors in these two regions respond to the momentum cycle in an anticorrelated sense.  The telescope is focused such that the PSF is sharpest at intermediate distances from the center of the FOV.  Since stars in the center and on the extreme edges have the blurriest PSFs \citep{VanCleve:2009}, they respond most strongly to the momentum cycle. 
 
 The mechanism behind the variability seen in $V_{2}$ is less clear.  $V_{2}$ includes a high frequency component with a period of 1.68 hours.  The \Kepler team has also noticed this periodicity in the pixel scale (Douglas Caldwell, private communication, 2012).  A possible explanation is thermal coupling of the telescope optics to a heater that turns off and on with a $\sim$20~minute period. The 1.68~hour variability would be an alias of this higher frequency with the observing cadence of 29.4~minutes.  The gradient in $a_{2}$ across the FOV suggests the heater is coupled to the telescope optics in a tip/tilt rather than piston sense.  
 
-The higher-order components $a_{3}$ and $a_{4}$ do not show significant spatial correlation, which suggests that $V_{3}$ and $V_{4}$ are not due to changes in the local PSF. Since $V_{3}$ and $V_{4}$ have a $\sim$10-day timescale, they could be the high frequency component of the DVA trend that was not removed by our 10-day spline.
+The higher-order components $a_{3}$ and $a_{4}$ do not show significant spatial correlation, which suggests that $V_{3}$ and $V_{4}$ are not due to changes in the local PSF. Since $V_{3}$ and $V_{4}$ have a $\sim$10-day timescale, they could be the high frequency component of the differential velocity aberration trend that was not removed by our 10-day spline.
 
 \begin{figure}
 \begin{center}
@@ -198,11 +205,11 @@ The RA and Dec positions of our 1000-star ensemble.  The points are color-coded
 \end{figure}
 
 \section{Removal of Modes}
-After determining which of the $N_{Mode}$ principle components correspond to noise modes, we can remove them according to Equation~\ref{eqn:fit}.  In Figure~\ref{fig:fits} we show fits to KIC-8144222 Q6 photometry using different combinations of TERRA principle components and PDC CBVs.  We fit for the PDC CBV coefficients using a linear least-squares minimizer.  We also show the fit using the \Kepler PDC module.
+After determining which of the $N_{Mode}$ principle components correspond to noise modes, we can remove them according to Equation~\ref{eqn:fit}.  In Figure~\ref{fig:fits} we show fits to KIC-8144222 Q6 photometry using different combinations of TERRA principle components and PDC CBVs.  We fit for the PDC CBV coefficients using a linear least squares minimizer.  We also show the fit using the \Kepler PDC algorithm.
 
 \begin{figure}
 \begin{center}
-\includegraphics{Fits.pdf}
+\plotone{fits.pdf}
 \end{center}
 \caption{
 Least squares fits using PDC (blue) and TERRA (red) principle components to KIC-8144222 Q6 photometry.  The bottom panel shows 12-hour $\mdf$ where smaller scatter implies greater sensitivity to small transits.  We show the spline fit (magenta) as a baseline since it incorporates no ensemble-based cotrending information.  The $\mdf$ using spline detrending shows large spikes at the momentum cycle cusps, which are suppressed in the TERRA and PDC cotrending.  Even after fitting 8 PDC CBVs, there is still considerable structure in the residuals.  The PDC module appears to be overfitting the photometry in order to account for the excursions at 570, 600, and 630 days.  This injects high frequency noise into regions of calibrated photometry that were featureless photometry calibrated with fewer CBVs.  Using our robust modes, we are able to produce a clean, calibrated light curve using only two modes.  Decreased model complexity helps guard against overfitting.
@@ -210,7 +217,7 @@ Least squares fits using PDC (blue) and TERRA (red) principle components to KIC-
 \label{fig:fits}
 \end{figure}
 
-Fits with 4 and 8 \Kepler CBVs show significant structure in the residuals.  We achieve more uniform residuals using only 2 of our modes.  The simplicity of our model buys some insurance against overfitting.  We believe that the high-frequency structure seen in the PDC light-curve is the result of overfitting, but we are unable to verify this because we do not have the PDC source code.  We believe that in an effort to reduce bulk global $\chi^{2}$, PDC chose mode weights that injected high-frequency noise into regions of calibrated photometry that were featureless in the 4 and 8 CBV fits.
+Fits with 4 and 8 \Kepler CBVs show significant structure in the residuals.  We achieve more uniform residuals using only 2 of our modes as we show quantitatively below.  The simplicity of our model buys some insurance against overfitting.  We believe that the high-frequency structure seen in the PDC light-curve is the result of overfitting, but we are unable to verify this because we do not have the PDC source code.  The tendency of the PDC algorithm to overfit photometry and inject high-frequency noise was the main motivation behind the improvements implemented in the PDC-MAP algorithm~\citep{Stumpe:2012}.  We believe that in an effort to reduce bulk global $\chi^{2}$, PDC chose mode weights that injected high-frequency noise into regions of calibrated photometry that were featureless in the 4 and 8 CBV fits.
 
 For each of the residuals in Figure~\ref{fig:fits}, we computed the mean depth $\mdf(t_{i})$ of a putative 12-hour transit centered at $t_{i}$ for every cadence in Q6.  The distribution of $\mdf$ due to noise determines the minimum transit depth that can be detected by a transit search algorithm.  $\mdf$ is computed by 
 \[
@@ -293,7 +300,7 @@ We computed the standard deviation, 90 percentile, and 99 percentile (in ppm) of
 \label{sec:conclusions}
 TERRA is a new technique for using ensemble photometry to self-calibrate instrumental systematics in \Kepler light curves.  We significantly reduce the complexity of our noise model by running a high-pass filter and removing thermal settling events before computing principle components.  TERRA's simplicity buys insurance against overfitting, a well-known shortcoming of the PDC algorithm.  For a typical $12.5 < $ \Kmag $ < 13.5$ and CDPP12 $< 40$~ppm star, TERRA achieves an additional $\sim$10~ppm suppression of peaks in $\mdf$ over PDC, allowing for the detection of smaller planets.
 
-The \Kepler PDC pipeline has evolved beyond that presented in \cite{Twicken:2010}.  The latest implementation, PDC-MAP \citep{Stumpe:2012,Smith:2012}, uses the ensemble of best fit coefficients, $a_{i}$, to establish a prior on the distribution of reasonable $a_{i}$.  If the best fit coefficients for a particular star are not consistent with the prior distribution, they relax to the prior.  PDC-MAP effectively tempers the tendency of the least-squares minimizer to overfit the photometry with unrealistic coefficients in an effort to reduce global $\chi^{2}$.  Our framework can easily incorporate and extend the MAP approach.  As seen Figure~\ref{fig:RADecCoeff}, some modes vary smoothly across the FOV.  Given that, we can construct a more narrow prior that is a function of position on the FOV.
+The \Kepler PDC pipeline has evolved beyond that presented in \cite{Twicken:2010}.  The latest implementation, PDC-MAP \citep{Stumpe:2012,Smith:2012}, uses the ensemble of best fit coefficients, $a_{i}$, to establish a prior on the distribution of reasonable $a_{i}$.  If the best fit coefficients for a particular star are not consistent with the prior distribution, they relax to the prior.  PDC-MAP effectively tempers the tendency of the least squares minimizer to overfit the photometry with unrealistic coefficients in an effort to reduce global $\chi^{2}$.  Our framework can easily incorporate and extend the MAP approach.  As seen Figure~\ref{fig:RADecCoeff}, some modes vary smoothly across the FOV.  Given that, we can construct a more narrow prior that is a function of position on the FOV.
 
 One feature in a future release of PDC is a multiscale approach to CBVs.  Multiscale PDC decomposes light curves in the wavelet domain before computing CBVs so that large scale features and small scale features are described by different CBVs \citep{Stumpe:2012multiscale}.  As we have shown, restricting the range of timescales present in the photometric ensemble allows for a cleaner separation of noise modes.
 
diff --git a/manuscript_hand.bib b/manuscript_hand.bib
index 3850952..8f942d6 100644
--- a/manuscript_hand.bib
+++ b/manuscript_hand.bib
@@ -47,6 +47,11 @@ year = {1943},
   url = "http://www.scipy.org/"
 }
 
-
+@Misc{KeplerArchiveManual,
+  author =    {D. Fraquelli and S. E. Thompson},
+  title =     {Kepler Archive Manual (KDMC-10008-004)},
+  year =      {2012},
+  url = "http://archive.stsci.edu/kepler/documents.html"
+}
 
 


==> texcmd.tex <==
\newcommand{\nThin}{847} % # of stars in Thin pop.
\newcommand{\nThick}{16} % # of stars in Thick pop.
\newcommand{\nHalo}{12} % # of stars in Halo pop.
\newcommand{\nBdr}{25} % # of stars in Bdr pop.
\newcommand{\nPop}{900} % # of stars with pop prob
\newcommand{\vsiniCutO}{7} % vsinicut for O
\newcommand{\teffCutOlo}{4700} % teff for O
\newcommand{\teffCutOhi}{6500} % teff for O
\newcommand{\maxTO}{0.11} % max temp correction O
\newcommand{\nStarsO}{694} % Number of stars with O analysis
\newcommand{\vsiniCutC}{15} % vsinicut for C
\newcommand{\teffCutClo}{5300} % teff for C
\newcommand{\teffCutChi}{6500} % teff for C
\newcommand{\maxTC}{0.15} % max temp correction C
\newcommand{\nStarsC}{704} % Number of stars with C analysis
\newcommand{\coThresh}{1.00} % Theshhold for high co
\newcommand{\scatterCut}{0.30} % Cut on the scatter
\newcommand{\teffSol}{5770} % Solar Effective Temp
\newcommand{\StdCompC}{0.09} 
\newcommand{\StdCompO}{0.08} 
\newcommand{\nCompC}{67}   
\newcommand{\nCompO}{16}   
\newcommand{\compCsigm}{0.00} % comp - C - sigm
\newcommand{\compCs}{0.17} % comp - C - s
\newcommand{\compCm}{0.08} % comp - C - m
\newcommand{\compCn}{625} % comp - C - n
\newcommand{\compFesigm}{0.00} % comp - Fe - sigm
\newcommand{\compFes}{0.27} % comp - Fe - s
\newcommand{\compFem}{0.06} % comp - Fe - m
\newcommand{\compFen}{970} % comp - Fe - n
\newcommand{\compOsigm}{0.00} % comp - O - sigm
\newcommand{\compOs}{0.14} % comp - O - s
\newcommand{\compOm}{0.05} % comp - O - m
\newcommand{\compOn}{606} % comp - O - n
\newcommand{\hostCsigm}{0.02} % host - C - sigm
\newcommand{\hostCs}{0.14} % host - C - s
\newcommand{\hostCm}{0.17} % host - C - m
\newcommand{\hostCn}{79} % host - C - n
\newcommand{\hostFesigm}{0.02} % host - Fe - sigm
\newcommand{\hostFes}{0.18} % host - Fe - s
\newcommand{\hostFem}{0.17} % host - Fe - m
\newcommand{\hostFen}{100} % host - Fe - n
\newcommand{\hostOsigm}{0.01} % host - O - sigm
\newcommand{\hostOs}{0.12} % host - O - s
\newcommand{\hostOm}{0.10} % host - O - m
\newcommand{\hostOn}{88} % host - O - n
\newcommand{\nStarsTot}{941} % 
\newcommand{\ncoGtThresh}{46} % 
\newcommand{\coMax}{1.55} % 
\newcommand{\ncoStarsTot}{457} % 
\newcommand{\coMin}{0.24} % 
\newcommand{\ncoLtThresh}{411} % 
\newcommand{\nPlanetTot}{97} % 

